MedCaseAgent: From Multimodal Clinical Evidence to Rare Disease Case Reports

Although Large Language Models (LLMs) have demonstrated potential in clinical documentation, generating the rigorous, evidence-based reasoning required for unprecedented, atypical, and rare disease case reports remains a significant challenge. We present MedCaseAgent, an end-to-end agentic reasoning paradigm that bridges this gap by synthesizing publication-quality reports from unstructured clinical notes. MedCaseAgent leverages a hierarchical structure, integrating patient-level data mining with iterative, tool-integrated reasoning. By dynamically querying medical literature and knowledge bases, the agent maintains high clinical fidelity and assesses case novelty. The framework is inherently modular, supporting various backbone LLMs in a plug-and-play fashion. To facilitate this research, we release MedCase-150K, a large-scale multimodal clinical case-report corpus, and MedCase-Bench, a robust temporally held-out evaluation suite. We also introduce an open-source model post-trained from Qwen3.5-9B and optimized specifically for this task. Under both LLM-judged and rule-based evaluation, MedCaseAgent outperforms existing general-purpose and specialized medical LLMs and agents. Blinded expert reviews and ablations further support the system's clinical relevance and evidence grounding.

==> Makefile <==
# Local build. On Overleaf this file is ignored; 00README.json drives the build.
#
#   make          build main.pdf (pdflatex -> bibtex -> pdflatex x2)
#   make quick    single pdflatex pass, for a fast look
#   make clean    remove build products
#   make cleanall also remove main.pdf

MAIN = main

all: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex $(wildcard sec/*.tex) $(wildcard tables/*.tex) $(MAIN).bib
	pdflatex -interaction=nonstopmode $(MAIN).tex
	-bibtex $(MAIN)
	pdflatex -interaction=nonstopmode $(MAIN).tex
	pdflatex -interaction=nonstopmode $(MAIN).tex

quick:
	pdflatex -interaction=nonstopmode $(MAIN).tex

clean:
	rm -f *.aux *.bbl *.blg *.log *.out *.toc *.ptc *.fls *.fdb_latexmk \
	      *.synctex.gz *.lof *.lot sec/*.aux

cleanall: clean
	rm -f $(MAIN).pdf

.PHONY: all quick clean cleanall

